Extending the practical applicability of the Kalman Filter

A Schmidt filter is a modification of the Kalman filter that allows to append system parameters as states and considers their uncertainty effect in the filtering process without attempting to estimate such parameters. The states that are only considered but not estimated, are generally known as \textit{consider} or \textit{considered} states. The main contributions of this research are the formulations of a Schmidt-Kalman filter that incorporates the numerical robustness of the well-known square root and factorized filtering forms plus the capacity of actively attempting to update the \textit{considered} states. The filters formulations proposed in this research are a fundamental extension of the Kalman filter. Therefore, the formulations of this work also apply within the Extended Kalman filter framework. More importantly, they are shown to handle nonlinearities, larger initial uncertainties, and poorly conditioned systems better than a typical Extended or Schmidt Kalman filter. Because the new filters are directly based on the Schmidt filter, they offer a novel and straight-forward filtering framework, allowing the use of a more simple filter where a more advanced or elaborated technique could have been needed.

==> data/Observability.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Humberto Ramos
%  Version 3.17.09
%  Last Updated: 11/30/2018
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                           SECTION II
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\chapter{U-D PARTIAL-UPDATE KALMAN FILTER}
\section{Motivation}
\section{Derivation of the factorized filter}
\section{Numerical examples: Stressing numerical and initial uncertainty filter robustness}
\subsection{Body reentring Earth atmosphere}
\subsection{Montecarlo results}
\subsection{Visual-aided inertial navigation}
\subsection{Montecarlo results}
\section{Comparing the Square root, UD filters, Joseph and conventional forms}
\subsection{Running time comparison}



==> data/TODO.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           TODO 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{TODO}

\indent 
\section{General notes}
\begin{enumerate}
	\item Use fuzzy logic to adapt weights.
	\item Is there an optimal way, in some sense, to pick the weights? Minimize non-linear effects? 
	\item The partial update works since it limits how aggressive (how fast the variables become correlated) the correlations between the variables is. It seems that it limits the speed at which the correlations are build before the filter tends to be inconsistent or to diverge.
	\item Partial update may be used for constraining states and assigning proper covariances.
	
\end{enumerate}

\textbf{Check Kalman Filtering : Theory and Practice Using MATLAB California State University at Fullerton pp 44.}

This book is very good at explaining stuff for linear stochastic systems. And actually, I got the idea of how to explain practical observability from it.

%\section{}
The fine mathematical assessment of the system observability, namely checking the rank of the observability matrix, can be affected by several factors including:

\begin{enumerate}
	\item Finite computation precision
	\item Truncation of the model
	\item Simple ignorance about system facts
\end{enumerate}

Read Kijubaran observability stuff, there is a good content there.

Also in the book Advanced Kalman Filtering, Least-Squares and Modeling there is an awesome discussion on how to use SVD to assess numerical observability. In this book there is even a tip on how to use QR decomposition for this.
\section{Spherical pendulum}
Some observations about the pendulum
\begin{enumerate}
	\item The model indicates that the momentum p1 needs to be conserved. This complicates the numerical stability of the simulation if: 1) The motion is small compared to the numerical noise of the simulation. It was observed that when small motions were imposed, the numerical errors are significant with respect to the motion. 2) The simulated measurement noise is very low. This provokes the system to get measurements that are almost exactly the propagated true states, which include numerical errors. If these very exact measurements are used in the filter, they could indicate an increase in values that are assumed to be constant, hence introduction of artificial energy is involuntary added to the system. Accumulation of this errors can cause the system to fail. In summary, we need good observability or good signal to (numerical) noise ratio.
\end{enumerate}



 


==> data/bibliography.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.
%
%  Author: Sean Zachary Roberson
%	 Version 3.16.09
%  Last updated 9/12/2016
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           REFERENCES 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phantomsection
\addcontentsline{toc}{chapter}{REFERENCES}

\renewcommand{\bibname}{{\normalsize\rm REFERENCES}}

%\bibliographystyle{ieeetr}
\bibliography{data/myReference}

==> data/nomenclature.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           NOMENCLATURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{NOMENCLATURE}
\addcontentsline{toc}{chapter}{NOMENCLATURE}  % Needs to be set to part, so the TOC doesnt add 'CHAPTER ' prefix in the TOC.

%A note about aligning: These entries will align
%themselves according to the ampersand (&).
%No extra spaces are needed, as seen in some of
%the entries below.

%Example of the longtable environment.
\hspace*{-1.25in}
\vspace{12pt}
\begin{spacing}{1.0}
	\begin{longtable}[htbp]{@{}p{0.35\textwidth} p{0.62\textwidth}@{}}
	   % \begin{tabular}{@{}p{0.33\textwidth} p{0.62\textwidth}@{}}
	    KF	&	Kalman filter\\	[2ex]
		EKF	&	Extended Kalman filter\\	[2ex]
		MEKF		&	Multiplicative Extended Kalman filter\\	[2ex]
		PU-MEKF	&	Partial-update Multiplicative Extended Kalman filter\\	[2ex] 
		UKF			&	Unscented Kalman filter\\	[2ex]
		PSKF & Partial-Update Schmidt Kalman filter\\ [2ex]
		UD & U and D factors\\ [2ex]
		DNL & Dynamic Nonlinearity-aware\\ [2ex]
		DC & Dynamic Covariance-aware\\ [2ex]
		PU & Partial-Update\\ [2ex]
		MC & Montecarlo\\ [2ex]
		UAV & Unmanned Air Vehicle\\ [2ex]
     	IMU & Inertial Measurement Unit\\ [2ex]
     	WMGS & Weighted Modified Gram-Schmidt\\ [2ex]
		%XXXXXXXX		&	This is an optional page. Random word to test how long the sentence can be? This is just for test purpose. The current setting aims to align left/right margin same as all other pages.\\	[2ex]
	   % \end{tabular}%
	\end{longtable}
\end{spacing}

\pagebreak{}

==> data/recommendations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\chapter{DYNAMIC UPDATE PRACTITIONER RECOMMENDATIONS}



